OMRA: Online Motion Resolution Adaptation to Remedy Domain Shift in Learned Hierarchical B-frame Coding

Learned hierarchical B-frame coding aims to leverage bi-directional reference frames for better coding efficiency. However, the domain shift between training and test scenarios due to dataset limitations poses a challenge. This issue arises from training the codec with small groups of pictures (GOP) but testing it on large GOPs. Specifically, the motion estimation network, when trained on small GOPs, is unable to handle large motion at test time, incurring a negative impact on compression performance. To mitigate the domain shift, we present an online motion resolution adaptation (OMRA) method. It adapts the spatial resolution of video frames on a per-frame basis to suit the capability of the motion estimation network in a pre-trained B-frame codec. Our OMRA is an online, inference technique. It need not re-train the codec and is readily applicable to existing B-frame codecs that adopt hierarchical bi-directional prediction. Experimental results show that OMRA significantly enhances the compression performance of two state-of-the-art learned B-frame codecs on commonly used datasets.

==> chapter/3-2_down8_warped.tex <==
\begin{figure}[t!]
    \begin{center}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_frame17_down8.png}
        \caption{}
        \label{fig:warp_d8}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_frame17_gt.png}
        \caption{}
        \label{fig:f17_gt}
    \end{subfigure}

    \caption{(a) Lowest temporal level warped frame generated by applying the flow obtained from down-sampled frames with a factor of 8. (b) Ground truth frame of the first temporal level frame. Generated flow using down-sampled input frames results in a higher-quality warped frame in fast video sequences.}
    \label{fig:down_factor_8}
    \end{center}
    \vspace{-1.5em}
\end{figure}

% Figure~\ref{fig:warp_d8} and~\ref{fig:f17_gt} depict the warped frames generated by the flow obtained from referenced frames down-sampled by a factor of 8 and the corresponding ground truth frame, respectively. Notably, the red box in Figure~\ref{fig:warp_d8} demonstrates that the player in the frame can be accurately predicted in the correct position, in contrast to Figure~\ref{fig:test_warp}, where a reasonable prediction about the frame cannot be achieved.


==> chapter/4-3_fast_visualizations.tex <==
\vspace{-3em}
\begin{figure}[t!]
    \begin{center}
    % \hfill
    % \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_frame1.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering Past ($x_{1}$)}
        \label{fig: ground_truth}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_frame_17_gt.png}
        \captionsetup{font=footnotesize}
        \caption{\centering Target ($x_{17}$)}
        \label{fig: ground_truth}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_frame33.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering Future ($x_{33}$)}
        \label{fig: ground_truth}
    \end{subfigure}


    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_warp_p_17_down8.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering $W(x_{1}, F_{17\to{1}})$ (MaskCRT + OMRA)}
        \label{fig:down 2}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_sys_17_down8.jpg}
        \captionsetup{font=footnotesize}
        \caption{\fontsize{7.95}{5}\selectfont \centering $\;\;\;mc^{(S)}_{17}\;\;\;$  \\(MaskCRT + OMRA)}
        \label{fig:down 8}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_warp_f_17_down8.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering $W(x_{33}, F_{17\to{33}})$ (MaskCRT + OMRA)}
        \label{fig:down 4}
        
    \end{subfigure}

    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_warp_p_17_down1.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering $W(x_{1}, F_{17\to{1}})$ (MaskCRT)}
        \label{fig:down 2}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_sys_17_down1.jpg}
        \captionsetup{font=footnotesize}
        \caption{\fontsize{7.95}{5}\selectfont \centering $\;\;\;mc^{(S)}_{17}\;\;\;$    (MaskCRT)}
        \label{fig:down 8}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/ba_vis_warp_f_17_down1.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering $W(x_{33}, F_{17\to{33}})$  (MaskCRT)}
        \label{fig:down 4}
    \end{subfigure}
    








    
    \caption{Visualization of the warped frames and temporal predictors in $BasketballDrive$. The first row is input frames, with (a)(c) being the reference frames and (b) the target frame. The second row is results with OMRA, where (d) and (f) are temporally warped frames from (a) and (c), respectively. (e) is the temporal predictor. Likewise, the third row is the corresponding results without OMRA. $W(x_t,F_{t \to t'})$ denotes backward warping, where $x_t$ is the reference frame to be warped and $F_{t \to t'}$ describes the backward flow from $x_t$ to $x_{t'}$.}
    \label{fig:ba_visualization}
    \end{center}
    \vspace{-1.5em}
\end{figure}

==> chapter/4-3_slow_visualizations.tex <==
\begin{figure}[t!]
    \begin{center}

    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/honey_vis_frame1.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering Past ($X_{1}$)}
        \label{fig: ground_truth}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/honey_frame_17_gt.png}
        \captionsetup{font=footnotesize}
        \caption{\centering Target ($X_{17}$)}
        \label{fig: ground_truth}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/honey_vis_frame33.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering Future ($X_{33}$)}
        \label{fig: ground_truth}
    \end{subfigure}

    % \begin{subfigure}{0.32\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figure/honey_vis_warp_p_17_down8.png}
    %     \caption{\centering $W(X_{1}, F_{17\to{1}})$ (\textcolor{blue}{w/ OMRA})}
    %     \label{fig:down 2}
    % \end{subfigure}
    % \begin{subfigure}{0.32\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figure/honey_vis_sys_17_down8.png}
    %     \caption{\centering synthesis frame    (\textcolor{blue}{w/ OMRA})}
    %     \label{fig:down 8}
    % \end{subfigure}
    % \begin{subfigure}{0.32\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figure/honey_vis_warp_f_17_down8.png}
    %     \caption{\centering $W(X_{33}, F_{17\to{33}})$ (\textcolor{blue}{w/ OMRA})}
    %     \label{fig:down 4}
    % \end{subfigure}

    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/honey_vis_warp_p_17_down8.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering $W(x_{1}, F_{17\to{1}})$ (MaskCRT + OMRA)}
        \label{fig:down 2}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/honey_vis_sys_17_down8.jpg}
        \captionsetup{font=footnotesize}
        \caption{\fontsize{7.95}{5}\selectfont \centering $\;\;\;mc^{(S)}_{17}\;\;\;$     (MaskCRT + OMRA)}
        \label{fig:down 8}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/honey_vis_warp_f_17_down8.jpg}
        \captionsetup{font=footnotesize}
        \caption{\centering $W(x_{33}, F_{17\to{33}})$ (MaskCRT + OMRA)}
        \label{fig:down 4}
    \end{subfigure}


    \begin{subfigure}{0.32\linewidth}
        \centering
        \captionsetup{font=footnotesize}
        \includegraphics[width=\linewidth]{figure/honey_vis_warp_p_17_down1.jpg}
        \caption{\centering $W(X_{1}, F_{17\to{1}})$ (MaskCRT)}
        \label{fig:down 2}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \captionsetup{font=footnotesize}
        \includegraphics[width=\linewidth]{figure/honey_vis_sys_17_down1.jpg}
        \caption{\fontsize{7.95}{5}\selectfont \centering $\;\;\;mc^{(S)}_{17}\;\;\;$     (MaskCRT)}
        \label{fig:down 8}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \captionsetup{font=footnotesize}
        \includegraphics[width=\linewidth]{figure/honey_vis_warp_f_17_down1.jpg}
        \caption{\centering $W(X_{33}, F_{17\to{33}})$  (MaskCRT)}
        \label{fig:down 4}
    \end{subfigure}
    





%     % \hfill
%     % \hfill





    
    \caption{Visualization of the warped frames and the temporal predictors for $HoneyBee$. All the notations follow the caption in Fig.~\ref{fig:ba_visualization}.}
    \label{fig:honey_visualization}
    \end{center}
    \vspace{-1.5em}
\end{figure}


% \begin{figure}[t!]
% \centering
% \resizebox{\textwidth}{!}
% {
% \begin{tabular}{ccc}

%     $x_t$ & $m \odot x_c$ & $ x_t - m \odot x_c$ \\

%     \includegraphics[width=0.3\textwidth]{figure/ba_vis_frame1.png}&
%     \includegraphics[width=0.3\textwidth]{figure/ba_vis_frame1.png}&
%     \includegraphics[width=0.3\textwidth]{figure/ba_vis_frame1.png}& \\

% \end{tabular}
% }

% \label{fig:visual}
% \end{figure}

==> table/BD_PWC.tex <==
\begin{table}[h]
    \centering
    \caption[]{BD-rate saving of two Motion Estimation networks.}
    % \vspace{\baselineskip}
    % \vspace{-0.7em}
    \normalsize 
    
    \begin{tabular}{cccc}
        \hline
        \multicolumn{4}{c}{\multirow{2}{*}{BD-rate (\%) PSNR-YUV}} \\\\
        \hline
          \multicolumn{1}{c}{\multirow{2}{*}{ME-network}} & \multicolumn{1}{c}{\multirow{2}{*}{UVG}} & \multicolumn{1}{c}{\multirow{2}{*}{HEVC-B}} & \multicolumn{1}{c}{\multirow{2}{*}{MCL-JCV}}  \\\\
        \hline
        \multicolumn{1}{c}{{SpyNet}}   &   \multicolumn{1}{c}{{-17.7}}   &   \multicolumn{1}{c}{{-11.0}}   &   \multicolumn{1}{c}{{-15.9}}   \\
         \multicolumn{1}{c}{{PWC-Net}}   &   \multicolumn{1}{c}{{-9.6}}   &   \multicolumn{1}{c}{{-6.3}}    &   \multicolumn{1}{c}{{-8.9}}
         \\\hline
         
    \end{tabular}
    \label{tab:BD_PWC}
    \vspace{-2em}
\end{table}

==> table/bdrate_4factor.tex <==
\begin{table}[htb]
\small
\centering
\caption{BD-rate comparison across different down-sampling factors applied to MaskCRT~\cite{maskCRT} in the HEVC-B dataset. The anchor is the inference always using full resolution input frames ($DF=1$), which is aligned with the result in MaskCRT. \textcolor{blue}{Not Sure about this aprt}}
\label{tab:bd_4factor}
\begin{tabular}{ccccc}
\hline
\multicolumn{5}{c}{BD-rate (\%) PSNR-RGB}                    \\ \hline
\multirow{2}{*}{Sequence} & \multicolumn{4}{c}{Scale Factor} \\ \cline{2-5} 
                          & 1     & 2      & 4      & 8      \\ \hline
BasketballDrive           & 0.00  & -12.4  & 9.21   & 79.43  \\
BQTerrace                 & 0.00  & 16.33  & 205.70 & 611.26 \\
Cactus                    & 0.00  & 10.05  & 119.48 & 362.69 \\
Kimono1                   & 0.00  & -9.27  & 0.05   & 31.21  \\
ParkScene                 & 0.00  & 6.59   & 100.11 & 431.51    \\ \hline
\end{tabular}
\end{table}



==> table/intra_period.tex <==
\begin{table}[t]
    \centering
    \caption[]{BD-rate comparison under Intra-Period 16 setting. The anchor models are B-CANF~\cite{bcanf}, MaskCRT~\cite{maskCRT} under an intra-period 16 setting.}
    % \vspace{\baselineskip}
    % \vspace{-0.7em}
    \small 
    
    \begin{tabular}{ccccc}
        \hline
        \multicolumn{5}{c}{\multirow{1}{*}{BD-rate (\%) PSNR-RGB}} \\
        \hline
          \multicolumn{1}{c}{\multirow{1}{*}{Method}} & & \multicolumn{1}{c}{\multirow{1}{*}{HEVC-B}} & \multicolumn{1}{c}{\multirow{1}{*}{UVG}} & \multicolumn{1}{c}{\multirow{1}{*}{MCL-JCV}}  \\
        \hline
        \multicolumn{1}{c}{{MaskCRT}}  &  &   \multicolumn{1}{c}{{0.00}}   &   \multicolumn{1}{c}{{0.00}}   &   \multicolumn{1}{c}{{0.00}}   \\
         \multicolumn{1}{c}{{MaskCRT + OMRA}}  &  &   \multicolumn{1}{c}{{-6.2}}   &   \multicolumn{1}{c}{{-12.4}}    &   \multicolumn{1}{c}{{-11.4}}
         \\\hline
         \multicolumn{1}{c}{{B-CANF}}  &  &   \multicolumn{1}{c}{{0.00}}   &   \multicolumn{1}{c}{{0.00}}   &   \multicolumn{1}{c}{{0.00}}   \\
         \multicolumn{1}{c}{{B-CANF + OMRA}} &   &   \multicolumn{1}{c}{{-3.4}}   &   \multicolumn{1}{c}{{-8.3}}    &   \multicolumn{1}{c}{{-6.0}}
         \\\hline
         
    \end{tabular}
    \label{tab:BD-rate_I16}
    \vspace{-1em}
\end{table}

==> table/three_variants_description.tex <==
\vspace{-0.5em}
\begin{table}[t]
    \centering
    \caption[]{Different variants of our frame-wise optimization method.}
    % \vspace{\baselineskip}
    % \vspace{-0.7em}
    \scriptsize
    
    \begin{tabular}{cc}
        \hline
        \multicolumn{1}{c}{\multirow{1}{*}{Settings}} & \multicolumn{1}{c}{\multirow{1}{*}{Scheme}}\\
        
        \hline
         % \multicolumn{1}{c}{Original MaskCRT} &   \multicolumn{1}{c}{0.0}  &   \multicolumn{1}{c}{0.0}   & \multicolumn{1}{c}{0.0}  \\
        \multicolumn{1}{c}{A}  & \multicolumn{1}{c}{Compress $\rightarrow$ Up\_Flow $\rightarrow$ Warp} \\ 
        
         \multicolumn{1}{c}{B}  &\multicolumn{1}{c}{Up\_Flow $\rightarrow$ Compress $\rightarrow$ Warp}\\
         
         \multicolumn{1}{c}{C}  &\multicolumn{1}{c}{Compress $\rightarrow$ Warp $\rightarrow$ Up\_MC} \\
            \hline

    \end{tabular}
    \label{tab:three_variants_description}
    % \vspace{-3em}
\end{table}
